MeshfreeFlowNet: A Physics-Constrained Deep Continuous Space-Time Super-Resolution Framework

We propose MeshfreeFlowNet, a novel deep learning-based super-resolution framework to generate continuous (grid-free) spatio-temporal solutions from the low-resolution inputs. While being computationally efficient, MeshfreeFlowNet accurately recovers the fine-scale quantities of interest. MeshfreeFlowNet allows for: (i) the output to be sampled at all spatio-temporal resolutions, (ii) a set of Partial Differential Equation (PDE) constraints to be imposed, and (iii) training on fixed-size inputs on arbitrarily sized spatio-temporal domains owing to its fully convolutional encoder. We empirically study the performance of MeshfreeFlowNet on the task of super-resolution of turbulent flows in the Rayleigh-Benard convection problem. Across a diverse set of evaluation metrics, we show that MeshfreeFlowNet significantly outperforms existing baselines. Furthermore, we provide a large scale implementation of MeshfreeFlowNet and show that it efficiently scales across large clusters, achieving 96.80% scaling efficiency on up to 128 GPUs and a training time of less than 4 minutes.

==> Sections/TitleAndAuthors.tex <==
\title{\alg: A Physics-Constrained Deep Continuous Space-Time Super-Resolution Framework}


\newif\ifprintauthors

%Comment this line to suppress printing authors
\printauthorstrue

\ifprintauthors
 \author{
 \IEEEauthorblockN{Chiyu ``Max" Jiang\IEEEauthorrefmark{1}\IEEEauthorrefmark{2}}
 \IEEEauthorblockA{%Mechanical Engineering\\
 %University of California\\
 %Berkeley, CA 94720, USA\\
 chiyu.jiang@berkeley.edu}\\
 \IEEEauthorblockN{Karthik Kashinath\IEEEauthorrefmark{3}}
 \IEEEauthorblockA{%NERSC\\
 %Lawrence Berkeley National Laboratory\\
 %Berkeley, CA 94720, USA\\
 kkashinath@lbl.gov}\\
 \IEEEauthorblockN{Philip Marcus\IEEEauthorrefmark{2}}
\IEEEauthorblockA{%Mechanical Engineering\\
 %University of California\\
 %Berkeley, CA 94720, USA\\
 pmarcus@me.berkeley.edu}\\
 \and
 \IEEEauthorblockN{Soheil Esmaeilzadeh\IEEEauthorrefmark{1}\IEEEauthorrefmark{4}}
 \IEEEauthorblockA{%Energy Resources Engineering\\
 %Stanford University\\
 %Stanford, CA 94305, USA\\
 soes@stanford.edu }\\
 \IEEEauthorblockN{Mustafa Mustafa\IEEEauthorrefmark{3}}
 \IEEEauthorblockA{%NERSC\\
 %Lawrence Berkeley National Laboratory\\
 %Berkeley, CA 94720, USA\\
 mmustafa@lbl.gov}\\
 \IEEEauthorblockN{Prabhat\IEEEauthorrefmark{3}}
 \IEEEauthorblockA{%NERSC\\
 %Lawrence Berkeley National Laboratory\\
 %Berkeley, CA 94720, USA\\
 prabhat@lbl.gov}\\
 \and
 \IEEEauthorblockN{Kamyar Azizzadenesheli\IEEEauthorrefmark{5}}
 \IEEEauthorblockA{%Department of Computing + Mathematical Sciences\\
 %California Institute of Technology\\
 %Pasadena, CA, 91125, USA\\
 kazizzad@caltech.edu}\\
 \IEEEauthorblockN{Hamdi A. Tchelepi\IEEEauthorrefmark{4}}
 \IEEEauthorblockA{%Energy Resources Engineering\\
 %Stanford University\\
 %Stanford, CA 94305, USA\\
 tchelepi@stanford.edu}\\
 \IEEEauthorblockN{Anima Anandkumar\IEEEauthorrefmark{5}\IEEEauthorrefmark{6}}
 \IEEEauthorblockA{%Energy Resources Engineering\\
 %Stanford University\\
 %Stanford, CA 94305, USA\\
 anima@caltech.edu}\\
 \thanks{\IEEEauthorrefmark{1}
 Denotes equal contribution.}
 \thanks{\IEEEauthorrefmark{2}
 University of California,
 Berkeley, CA 94720, USA}
 \thanks{\IEEEauthorrefmark{3}
 Lawrence Berkeley National Laboratory,
 Berkeley, CA 94720, USA}
 \thanks{\IEEEauthorrefmark{4}
 Stanford University,
 Stanford, CA 94305, USA}
 \thanks{\IEEEauthorrefmark{5}
 California Institute of Technology,
 Pasadena, CA, 91125, USA}
 \thanks{\IEEEauthorrefmark{6}
 NVIDIA, 
 Santa Clara, CA 95051, USA}
 }
 
 
%  \author{
% \IEEEauthorblockN{Chiyu ``Max" Jiang\IEEEauthorrefmark{1}}
%  \IEEEauthorblockA{%Mechanical Engineering\\
%  %University of California\\
%  %Berkeley, CA 94720, USA\\
%  chiyu.jiang@berkeley.edu}\\
%  \IEEEauthorblockN{Soheil Esmaeilzadeh\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%Energy Resources Engineering\\
%  %Stanford University\\
%  %Stanford, CA 94305, USA\\
%  soes@stanford.edu }\\
%   \IEEEauthorblockN{Azizzadenesheli\IEEEauthorrefmark{3}}
%  \IEEEauthorblockA{%Department of Computing + Mathematical Sciences\\
%  %California Institute of Technology\\
%  %Pasadena, CA, 91125, USA\\
%  kazizzad@caltech.edu}\\
%  \IEEEauthorblockN{Karthik Kashinath\IEEEauthorrefmark{4}}
%  \IEEEauthorblockA{%NERSC\\
%  %Lawrence Berkeley National Laboratory\\
%  %Berkeley, CA 94720, USA\\
%  kkashinath@lbl.gov}\\
%  \and 
%  \IEEEauthorblockN{Sean Treichler\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%\\
%  \thanks{\IEEEauthorrefmark{2}
%  NVIDIA,
%  Santa Clara, CA 95051, USA }
%  sean@nvidia.com}\\
%  \IEEEauthorblockN{Everett Phillips\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%NVIDIA\\
%  %Santa Clara, CA 95051, USA\\
%  ephillips@nvidia.com}\\
%  \IEEEauthorblockN{Massimiliano Fatica\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%NVIDIA\\
%  %Santa Clara, CA 95051, USA\\
%  mfatica@nvidia.com}\\
%  \and
%  \IEEEauthorblockN{Joshua Romero\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%NVIDIA\\
%  %Santa Clara, CA 95051, USA\\
%  joshr@nvidia.com} \\
%  \IEEEauthorblockN{Ankur Mahesh\IEEEauthorrefmark{1}}
%  \IEEEauthorblockA{%NERSC\\
%  %Lawrence Berkeley National Laboratory\\
%  %Berkeley, CA, 94720, USA\\
%  amahesh@lbl.gov}\\
%  \IEEEauthorblockN{Prabhat\IEEEauthorrefmark{1}}
%  \IEEEauthorblockA{%NERSC\\
%  %Lawrence Berkeley National Laboratory\\
%  %Berkeley, CA 94720, USA\\
%  prabhat@lbl.gov} \\
%  \and
%  \IEEEauthorblockN{Mayur Mudigonda\IEEEauthorrefmark{1}}
%  \IEEEauthorblockA{%NERSC\\
%  %Lawrence Berkeley National Laboratory\\
%  %Berkeley, CA 94720, USA\\
%  mudigonda@berkeley.edu}\\
%  \IEEEauthorblockN{Michael Matheson\IEEEauthorrefmark{3}}
%  \IEEEauthorblockA{%\\
%  \thanks{\IEEEauthorrefmark{3}
%  Oak Ridge National Laboratory,
%  Oak Ridge, TN 37831, USA }
%  mathesonma@ornl.gov}\\
%  \IEEEauthorblockN{Michael Houston\IEEEauthorrefmark{2}}
%  \IEEEauthorblockA{%NVIDIA\\
%  %Santa Clara, CA 95051, USA\\
%  mhouston@nvidia.com} \\
%  }
 \IEEEaftertitletext{\vspace{-1cm}}
\fi

==> Tables/tab-noise.tex <==
\renewcommand{\arraystretch}{1}
\begin{table*}[h!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|ccccccccc|c}
& \multicolumn{9}{c|}{\makecell{100$\times$NMAE\\(R2)}}                                       & \multicolumn{1}{c}{} \\
\makecell{Dataset} & $E_{tot}$ & $u_{rms}$ & $\varepsilon$ & $\lambda$ & $Re_{\lambda}$ & $\tau_{\eta}$ & $\eta$ & $L$ & $T_L$ & avg. R2 \\ \hline
Clean &\makecell{0.698\\(0.9990)}    &\makecell{{0.666}\\(0.9987)}   &\makecell{{0.671}\\(0.9989)}   &\makecell{{0.554}\\(0.9983)}   &\makecell{{0.408}\\(0.9991)}   &\makecell{{0.805}\\(0.9971)}  &\makecell{{0.767}\\(0.9978)}   &\makecell{1.048\\(0.9946)}   &\makecell{{0.515}\\(0.9992)}   &0.9981                      \\ \cline{1-1}
Noisy &
       \makecell{{3.874}\\(0.9470)}&\makecell{{8.755}\\(0.8904)}&
       \makecell{{3.718}\\(0.9498)}&\makecell{{9.481}\\(0.8316)}&
       \makecell{{8.0351}\\(0.8367)}&\makecell{{10.783}\\(0.8351)}&
       \makecell{{10.234}\\(0.8584)}&\makecell{{4.582}\\(0.9440)}&
       \makecell{{5.073}\\(0.8642)}& {0.8841}                     
\end{tabular}
}
\vspace{1 pt}
\caption{For a \alg model that has been trained on one clean dataset, the super-resolution performance evaluation is respectively reported for clean and noisy coarse datasets with un-seen initial conditions. In the noisy dataset, a Gaussian noise with zero mean and unity standard deviation has been added in the normalized space of the physical parameters to the spatial coarse scale information at each time frame.}
\label{table:noisydata}
\end{table*}

